Deploying a Top-100 Supercomputer for Large Parallel Workloads: the Niagara Supercomputer

Niagara is currently the fastest supercomputer accessible to academics in Canada. It was deployed at the beginning of 2018 and has been serving the research community ever since. This homogeneous 60,000-core cluster, owned by the University of Toronto and operated by SciNet, was intended to enable large parallel jobs and has a measured performance of 3.02 petaflops, debuting at #53 in the June 2018 TOP500 list. It was designed to optimize throughput of a range of scientific codes running at scale, energy efficiency, and network and storage performance and capacity. It replaced two systems that SciNet operated for over 8 years, the Tightly Coupled System (TCS) and the General Purpose Cluster (GPC). In this paper we describe the transition process from these two systems, the procurement and deployment processes, as well as the unique features that make Niagara a one-of-a-kind machine in Canada.

==> Makefile <==
NAME=NIAGARA-pearc19
TARGET=$(NAME).pdf
SOURCE=$(NAME).tex

NAMEa=$(NAME)-extAbs
TARGETa=$(NAME)-extAbs.pdf
SOURCEa=$(NAME)-extAbs.tex

JUNK=.aux .bbl .blg .dvi .log .nav .out .ps .pdf .snm .tex.backup .tex.bak .toc Notes.bib .spl

.PHONY: clean


$(TARGET): $(SOURCE) *tex
	@pdflatex $(SOURCE)
	@bibtex $(NAME)
	@pdflatex $(SOURCE)
	@pdflatex $(SOURCE)

$(TARGETa): $(SOURCEa) *tex
	@pdflatex $(SOURCEa)
	@bibtex $(NAMEa)
	@pdflatex $(SOURCEa)
	@pdflatex $(SOURCEa)

all: $(TARGET) $(TARGETa)

abs: $(TARGETa)

full: $(TARGET)

clean:
	@for ext in $(JUNK); do \
		rm -v $(NAME)$$ext; \
		rm -v $(NAMEa)$$ext; \
	done

